Robust Attack Graph Generation

We present a method to learn automaton models that are more robust to input modifications. It iteratively aligns sequences to a learned model, modifies the sequences to their aligned versions, and re-learns the model. Automaton learning algorithms are typically very good at modeling the frequent behavior of a software system. Our solution can be used to also learn the behavior present in infrequent sequences, as these will be aligned to the frequent ones represented by the model. We apply our method to the SAGE tool for modeling attacker behavior from intrusion alerts. In experiments, we demonstrate that our algorithm learns models that can handle noise such as added and removed symbols from sequences. Furthermore, it learns more concise models that fit better to the training data.

==> code/fix_matched_sequence.tex <==
%!TEX root = ../report.tex

\begin{fullwidth}[width=\linewidth+1cm]

\begin{algorithm2e}[H]
    \AlgorithmSetup

    \SetKw{Skipped}{SKIPPED}
    \SetKw{Added}{ADDED}
    \SetKw{Jump}{JUMP}
    \SetKw{source}{source}
    \SetKw{target}{target}
    \SetKw{name}{name}


    \KwIn{edges: $E$}
    \KwOut{matched sequence: $S$}
    \BlankLine

    $S = [ ]$\;
    $i = 0$\;
    \While{$i < \Len($E$)$}{
        $edge = E[i]$\;
        $i = i + 1$\;
        \If{$\type(edge) == \Skipped$} {
            $last\_edge = S[-1]$\;
            \While{$\type(E[i]) == \Skipped$} {
                $i = i + 1$\;
            }
            $new\_edge = (\source=last\_edge.\target, \target=E[i].\target, \name = E[i].\name)$\;
            $S.\Append(new\_edge)$\;
        }
        % \ElseIf{$\type(edge) == \Added$}{
        %     $S.\Append(edge)$\;
        % }
        \Else{
            $S.\Append(edge)$\;
        }
    }

    \caption{Create the \textit{matched} sequence from the alignment output}
    \label{code:fix-matched-sequence}
\end{algorithm2e}
\end{fullwidth}

==> code/needleman_wunsch.tex <==
%!TEX root = ../report.tex

\begin{algorithm}[H]
\AlgorithmSetup
\SetKwFunction{MatchScore}{MatchScore}

 \KwIn{size of sequences: $m, n$}
 \KwOut{matrix: $M$}
 \For{$i = 0 \KwTo m$}{
  $M[i][0] =  GAP * i$\;
 }
 \For{$j = 0 \KwTo n$}{
  $M[0][j] =  GAP * j$\;
 }

 \For{$i = 1 \KwTo m$}{
  \For{$j = 1 \KwTo n$}{
    $match = M[i-1][j-1] + \MatchScore(x_i, y_j)$\;
    $delete = M[i-1][j] + GAP$\;
    $insert = M[i][j-1] + GAP$\;
    $M[i][j] = $ $\Max(match, delete, insert)$\;
  }
 }
 \caption{Needleman-Wunsch algorithm for sequence alignment. The \texttt{MatchScore} function returns \textit{MATCH} if the two arguments are equal, or \textit{MISMATCH} if not.}
 \label{code:needleman-wunsch}
\end{algorithm}


==> code/sage_backtracking.tex <==
%!TEX root = ../report.tex

\begin{algorithm2e}[htbp]
    \AlgorithmSetup

    \SetKwFunction{getMaxEdgeOfColumn}{getMaxEdgeOfColumn}
    \SetKwFunction{multipleMaxInRow}{multipleMaxInRow}
    \SetKwFunction{findAddedEdges}{findAddedEdges}
    \SetKwFunction{getSourceTarget}{getSourceTarget}
    \SetKwFunction{findPath}{findPath}
    \SetKwFunction{JumpEdge}{JumpEdge}
    \LinesNumbered

    \KwIn{alignment matrix: $M$, trace: $T$}
    \KwOut{aligned sequence: $S$}

    \For{$i = \Len(T) - 1 \KwTo 0$}{
        $edge$ = \getMaxEdgeOfColumn($M$, $i$)\;

        \If{\multipleMaxInRow($M, edge$)}{
            $S.\Append(\findAddedEdges(M, edge))$\;
        }\Else{
            $S.\Append(edge)$\;
        }
        \If{$\Len(S) \geq 2$}{
            $source, target = \getSourceTarget(S)$\;
            \If{$source \neq target$}{
                $skipped\_edges = \findPath(source, target)$\;
                \If{$skipped\_edges \neq []$} {
			        $S.\Append(skipped\_edges)$\;
                } \Else{
                    $j = \JumpEdge(source, target)$\;
                    $S.\Append(j)$\;
                }
            }
        }
    }


    \caption{Backtracing through the matrix to find the best alignment.}
    \label{code:sage-backtracking}
\end{algorithm2e}



==> code/ts_matrix.tex <==
%!TEX root = ../report.tex

\begin{algorithm}[h]
\AlgorithmSetup
\SetKwFunction{MatchScore}{MatchScore}
\SetKwFunction{GetThreeNeighbouringCells}{GetThreeNeighbouringCells}
\SetKwFunction{FindUpIndex}{FindUpIndex}
\KwIn{edges: $E$, trace: $T$}
\KwOut{alignment matrix: $M$}

\Fn{\GetThreeNeighbouringCells(i, j, edge, transition)}{
	$upIndex = \FindUpIndex(edge, i, j)$\;

	$left = M[i, j-1] + GAP$\;
	$up = M[upIndex, j] + GAP$\;
	$diagonal = M[upIndex, j-1] + \MatchScore(edge.label, transition)$\;
	\Return{[left, up, diagonal]}
}

$m = \Len(E)$\;
$n = \Len(T)$\;
\For{$edge \KwInOf E$}{
	$M[i][0] =  GAP * edge.level$\;
}
\For{$j = 0 \KwTo n$}{
	$M[0][j] =  GAP * j$\;
}

\For{$i = 1 \KwTo m$}{
	\For{$j = 1 \KwTo n$}{
		$edge = E[i]$\;
		$transitionLabel = T[j]$\;
		$neighbouringCells = \GetThreeNeighbouringCells(i, j, edge, transitionLabel)$\;
		$M[i][j] = \Max(neighbouringCells)$\;
	}
}


 \caption{Initialize and fill alignment matrix}
 \label{code:ts-matrix}
\end{algorithm}



==> figures/fix_path_cases.tex <==
\begin{figure}[t]
\floatconts
  {fig:matched-sequence-cases}
  {\caption{Example situations to make a matched sequence. In both subfigures, the left part is transformed into the right part.}}
  {%
    \subfigure[A combination of a single skipped and added edge get transformed into an edge with the added edge's label (a).]{\label{fig:skipped_added}%
      \begin{tikzpicture}[scale=0.14]
            \tikzstyle{every node}+=[inner sep=0pt]
            \draw [black] (23.8,-13.7) circle (3);
            \draw [black] (23.8,-24.3) circle (3);
            \draw [black] (41.6,-13.7) circle (3);
            \draw [black] (41.6,-24.3) circle (3);
            \draw [black] (22.169,-21.806) arc (-158.19728:-201.80272:7.554);
            \fill [black] (22.17,-21.81) -- (22.34,-20.88) -- (21.41,-21.25);
            \draw (21.13,-19) node [left] {b (skipped)};
            \draw [black] (25.192,-16.34) arc (17.88374:-17.88374:8.661);
            \fill [black] (25.19,-21.66) -- (25.91,-21.05) -- (24.96,-20.74);
            \draw (26.11,-19) node [right] {a (added)};
            \draw [black] (41.6,-16.7) -- (41.6,-21.3);
            \draw (42.4,-19) node [right] {a};
            \fill [black] (41.6,-21.3) -- (42.1,-20.5) -- (41.1,-20.5);
        \end{tikzpicture}}%
    \qquad
    \subfigure[Multiple skipped edges.]{\label{fig:skipped_multiple}%
      \begin{tikzpicture}[scale=0.14]
            \tikzstyle{every node}+=[inner sep=0pt]
            \draw [black] (23.8,-13.7) circle (3);
            \draw [black] (23.8,-24.3) circle (3);
            \draw [black] (43.9,-13.7) circle (3);
            \draw [black] (43.9,-35.2) circle (3);
            \draw [black] (23.8,-35.2) circle (3);
            \draw [black] (43.9,-24.3) circle (3);
            \draw [black] (23.8,-16.7) -- (23.8,-21.3);
            \fill [black] (23.8,-21.3) -- (24.3,-20.5) -- (23.3,-20.5);
            \draw (23.3,-19) node [left] {b (skipped)};
            \draw [black] (25.437,-26.792) arc (22.28205:-22.28205:7.801);
            \fill [black] (25.44,-32.71) -- (26.2,-32.16) -- (25.28,-31.78);
            \draw (26.52,-29.75) node [right] {a (added)};
            \draw [black] (22.362,-32.584) arc (-161.04396:-198.95604:8.725);
            \fill [black] (22.36,-32.58) -- (22.57,-31.67) -- (21.63,-31.99);
            \draw (21.39,-29.75) node [left] {b (skipped)};
            \draw [black] (46.318,-15.463) arc (46.9166:-46.9166:12.305);
            \fill [black] (46.32,-33.44) -- (47.24,-33.26) -- (46.56,-32.53);
            \draw (51,-24.45) node [right] {a};
        \end{tikzpicture}}
  }
\end{figure}

==> figures/results/cptc_2018_results_table.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
        \hline
        test case & number of tests & accuracy                             \\ \hline
        REMOVE-1  & 531              & \cellcolor[HTML]{C0C0C0}\textbf{1.0} \\ \hline
        REMOVE-2  & 2137             & \cellcolor[HTML]{C0C0C0}\textbf{1.0} \\ \hline
        ADD-1     & 531              & \cellcolor[HTML]{C0C0C0}\textbf{1.0}  \\ \hline
        ADD-2     & 109             & \cellcolor[HTML]{C0C0C0}\textbf{1.0}      \\ \hline
        SWAP-1    & 436              & \cellcolor[HTML]{C0C0C0}\textbf{0.93}  \\ \hline
        MODIFY-1  & 531              & \cellcolor[HTML]{C0C0C0}\textbf{1.0}  \\ \hline
        MODIFY-2  & 2137             & \cellcolor[HTML]{C0C0C0}\textbf{0.97}      \\ \hline
    \end{tabular}
    \caption{Results for the validation experiments of the CPTC-2018 dataset.}
    \label{tab:cptc-2018-results}
\end{table}

==> figures/results/synthetic_results_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
        \hline
        test case & number of tests & accuracy                             \\ \hline
        REMOVE-1  & 58              & \cellcolor[HTML]{C0C0C0}\textbf{100\%} \\ \hline
        REMOVE-2  & 109             & \cellcolor[HTML]{C0C0C0}\textbf{100\%} \\ \hline
        ADD-1     & 58              & \cellcolor[HTML]{C0C0C0}\textbf{90\%}  \\ \hline
        ADD-2     & 109             & \cellcolor[HTML]{C0C0C0}\textbf{87\%}      \\ \hline
        SWAP-1    & 38              & \cellcolor[HTML]{C0C0C0}\textbf{90\%}  \\ \hline
        MODIFY-1  & 58              & \cellcolor[HTML]{C0C0C0}\textbf{97\%}  \\ \hline
        MODIFY-2  & 109             & \cellcolor[HTML]{C0C0C0}\textbf{TODO}      \\ \hline
    \end{tabular}
    \caption{Results for the synthetic dataset.}
    \label{tab:synthetic-results}
\end{table}

==> figures/tables/iterative_results.tex <==
%!TEX root = ../../report.tex


\begin{table}[h!]
\makebox[\textwidth][c]{
\begin{tabular}{|r|c|c|c|c|c|r|r|r|r|}
\hline
Index & A                              & B                              & C                              & D                              & E               & Avg. Score & Std. Score & Avg. Size & Std. Size     \\ \hline
1 &\cellcolor[HTML]{E67C73}\textbf{FALSE} & \cellcolor[HTML]{57BB8A}\textbf{TRUE} & \cellcolor[HTML]{E67C73}\textbf{FALSE}    & \cellcolor[HTML]{57BB8A}\textbf{TRUE} & \cellcolor[HTML]{E67C73}\textbf{FALSE}    & \textbf{0.706}  & \textbf{0.014} & \textbf{131.3}   & \textbf{8.825} \\ \hline
2 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & 0.703 & 0.016 & 146.2 & 5.757  \\ \hline
3 &\cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & 0.699 & 0.019 & 138.7 & 5.617  \\ \hline
4 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & 0.699 & 0.029 & 143.8 & 4.810  \\ \hline
5 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & 0.694 & 0.022 & 136.0 & 4.933  \\ \hline
6 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & 0.693 & 0.038 & 136.8 & 13.359 \\ \hline
7 &\cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & 0.692 & 0.008 & 137.8 & 8.572  \\ \hline
8 &\cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & 0.691 & 0.019 & 135.5 & 15.229 \\ \hline
9 &\cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & 0.690 & 0.018 & 134.8 & 9.227  \\ \hline
10 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{57BB8A} TRUE  & \cellcolor[HTML]{E67C73} FALSE & 0.687 & 0.011 & 140.0 & 11.299 \\ \hline
28 &\cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & \cellcolor[HTML]{E67C73} FALSE & 0.662 & 0.025 & 119.7 & 6.80   \\ \hline
\end{tabular}
}
\caption{TODO}
\label{tab:iterative-results-top-10}
\end{table}

==> figures/tables/results-top10-linear.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
MATCH & MISMATCH & GAP & Accuracy \\ \hline
5 & -7  & -6  & 0.97 \\ \hline
5 & -7  & -5  & 0.97 \\ \hline
3 & -10 & -7  & 0.96 \\ \hline
3 & -8  & -4  & 0.96 \\ \hline
3 & -7  & -5  & 0.96 \\ \hline
3 & -6  & -5  & 0.96 \\ \hline
3 & -6  & -4  & 0.96 \\ \hline
5 & -10 & -10 & 0.96 \\ \hline
5 & -10 & -9  & 0.96 \\ \hline
5 & -10 & -8  & 0.96 \\ \hline
\end{tabular}
\caption{Top 10 results for Affine scoring and test case \textbf{ADD-1}.}
\label{tab:results-linear-add-1-top10}
\end{table}




\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
MATCH & MISMATCH & GAP & Accuracy \\ \hline
3     & -8       & -3  & 0.89     \\ \hline
4     & -9       & -4  & 0.89     \\ \hline
5     & -6       & -5  & 0.88     \\ \hline
3     & -5       & -3  & 0.88     \\ \hline
3     & -6       & -3  & 0.88     \\ \hline
4     & -7       & -4  & 0.88     \\ \hline
5     & -10      & -5  & 0.88     \\ \hline
4     & -10      & -4  & 0.88     \\ \hline
3     & -4       & -3  & 0.87     \\ \hline
4     & -5       & -4  & 0.87     \\ \hline
\end{tabular}
\caption{Top 10 results for Affine scoring and test case \textbf{ADD-2}.}
\label{tab:results-linear-add-2-top10}
\end{table}

==> figures/visual_analysis/merged_paths_1.tex <==
% \begin{figure}[htbp]
% \centering
% \subcaptionbox{Attack paths in original model\label{fig:merged-paths-1-a}}
% {
% \includegraphics[height=300pt]{figures/visual_analysis/dot_merged_paths_A.dot.png}
% } %
% % \hfill %
% \subcaptionbox{Attack paths in iterated model \label{fig:merged-paths-1-b}}
% {
% \includegraphics[height=300pt]{figures/visual_analysis/dot_merged_paths_B.dot.png}
% } %

% \caption{Nodes 1 and 3 have been merged in the iterative model, as the training sequences are very similar.}
% \label{fig:merged-paths-1}
% \end{figure}


\begin{figure}[htbp]
\floatconts
  {fig:merged-paths-1}
  {\caption{Nodes 1 and 3 have been merged in the iterative model, as the training sequences are very similar.}}
  {%
    \subfigure[Attack paths in original model. ]{\label{fig:merged-paths-1-a}%
        \includegraphics[height=280pt]{figures/visual_analysis/dot_merged_paths_A.dot}
    }
    \qquad \qquad \quad
    \subfigure[Attack paths in iterated SAAT model.]{\label{fig:merged-paths-1-b}%
        \includegraphics[height=280pt]{figures/visual_analysis/dot_merged_paths_B.dot}
    }
  }
\end{figure}

==> figures/visual_analysis/merged_paths_2.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:merged-paths-2}
  {\caption{Differences in attack paths in original and iterated model.}}
  {%
  \makebox[\textwidth][c]{
    \subfigure[Attack Paths in original model.]{\label{fig:merged-paths-2-a}%
      \begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (37.1,-0.5) circle (3);
\draw (37.1,-0.5) node {$0$};
\draw [black] (29.7,-6.3) circle (3);
\draw (29.7,-6.3) node {$1$};
\draw [black] (44.9,-6.3) circle (3);
\draw (44.9,-6.3) node {$2$};
\draw [black] (44.9,-16.1) circle (3);
\draw (44.9,-16.1) node {$3$};
\draw [black] (44.9,-26) circle (3);
\draw (44.9,-26) node {$4$};
\draw [black] (29.7,-16.1) circle (3);
\draw (29.7,-16.1) node {$8$};
\draw [black] (44.9,-35.6) circle (3);
\draw (44.9,-35.6) node {$5$};
\draw [black] (44.9,-45.7) circle (3);
\draw (44.9,-45.7) node {$6$};
\draw [black] (44.9,-55.5) circle (3);
\draw (44.9,-55.5) node {$7$};
\draw [black] (34.74,-2.35) -- (32.06,-4.45);
\fill [black] (32.06,-4.45) -- (33,-4.35) -- (32.38,-3.56);
\draw (20.47,-2.9) node [above] {bfCred|unassigned};
\draw [black] (39.51,-2.29) -- (42.49,-4.51);
\fill [black] (42.49,-4.51) -- (42.15,-3.63) -- (41.55,-4.43);
\draw (51,-2.9) node [above] {netDOS|http(s)};
\draw [black] (44.9,-9.3) -- (44.9,-13.1);
\fill [black] (44.9,-13.1) -- (45.4,-12.3) -- (44.4,-12.3);
\draw (45.4,-11.2) node [right] {infoD|http(s)};
\draw [black] (44.9,-19.1) -- (44.9,-23);
\fill [black] (44.9,-23) -- (45.4,-22.2) -- (44.4,-22.2);
\draw (45.4,-21.05) node [right] {surf|http(s)};
\draw [black] (29.7,-9.3) -- (29.7,-13.1);
\fill [black] (29.7,-13.1) -- (30.2,-12.3) -- (29.2,-12.3);
\draw (29.2,-11.2) node [left] {vulnD|storage};
\draw [black] (44.9,-29) -- (44.9,-32.6);
\fill [black] (44.9,-32.6) -- (45.4,-31.8) -- (44.4,-31.8);
\draw (45.4,-30.8) node [right] {vulnD|storage};
\draw [black] (44.9,-38.6) -- (44.9,-42.7);
\fill [black] (44.9,-42.7) -- (45.4,-41.9) -- (44.4,-41.9);
\draw (45.4,-40.65) node [right] {serD|unassigned};
\draw [black] (44.9,-48.7) -- (44.9,-52.5);
\fill [black] (44.9,-52.5) -- (45.4,-51.7) -- (44.4,-51.7);
\draw (45.4,-50.6) node [right] {hostD|http(s)};
\end{tikzpicture}}%
    \quad
    \subfigure[Attack paths in iterated model]{\label{fig:merged-paths-2-b}%
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (37.5,-5.3) circle (3);
\draw (37.5,-5.3) node {$0$};
\draw [black] (29.7,-13.1) circle (3);
\draw (29.7,-13.1) node {$1$};
\draw [black] (44.9,-13.1) circle (3);
\draw (44.9,-13.1) node {$2$};
\draw [black] (44.9,-22.9) circle (3);
\draw (44.9,-22.9) node {$3$};
\draw [black] (44.9,-32.6) circle (3);
\draw (44.9,-32.6) node {$4$};
\draw [black] (29.7,-38.3) circle (3);
\draw (29.7,-38.3) node {$5$};
\draw [black] (29.7,-48.3) circle (3);
\draw (29.7,-48.3) node {$6$};
\draw [black] (29.7,-59.3) circle (3);
\draw (29.7,-59.3) node {$7$};
\draw [black] (35.38,-7.42) -- (31.82,-10.98);
\fill [black] (31.82,-10.98) -- (32.74,-10.77) -- (32.03,-10.06);
\draw (21.66,-8.72) node [above] {bfCred|unassigned};
\draw [black] (39.56,-7.48) -- (42.84,-10.92);
\fill [black] (42.84,-10.92) -- (42.65,-10) -- (41.92,-10.69);
\draw (41.73,-7.73) node [right] {netDOS|http(s)};
\draw [black] (44.9,-16.1) -- (44.9,-19.9);
\fill [black] (44.9,-19.9) -- (45.4,-19.1) -- (44.4,-19.1);
\draw (45.4,-18) node [right] {infoD|http(s)};
\draw [black] (44.9,-25.9) -- (44.9,-29.6);
\fill [black] (44.9,-29.6) -- (45.4,-28.8) -- (44.4,-28.8);
\draw (45.4,-27.75) node [right] {surf|http(s)};
\draw [black] (42.09,-33.65) -- (32.51,-37.25);
\fill [black] (32.51,-37.25) -- (33.43,-37.43) -- (33.08,-36.5);
\draw (43,-36.09) node [below] {vulnD|storage};
\draw [black] (29.7,-16.1) -- (29.7,-35.3);
\fill [black] (29.7,-35.3) -- (30.2,-34.5) -- (29.2,-34.5);
\draw (29.2,-25.7) node [left] {vulnD|storage};
\draw [black] (29.7,-41.3) -- (29.7,-45.3);
\fill [black] (29.7,-45.3) -- (30.2,-44.5) -- (29.2,-44.5);
\draw (29.2,-43.3) node [left] {serD|unassigned};
\draw [black] (29.7,-51.3) -- (29.7,-56.3);
\fill [black] (29.7,-56.3) -- (30.2,-55.5) -- (29.2,-55.5);
\draw (30.2,-53.8) node [right] {hostD|http(s)};
\end{tikzpicture}}
  }%
 }
\end{figure}




% \begin{figure}[htbp]
% \centering
% \subcaptionbox{Attack Paths in original model.\label{fig:merged-paths-2-a}}
% {
% \begin{tikzpicture}[scale=0.12]
% \tikzstyle{every node}+=[inner sep=0pt]
% \draw [black] (37.1,-0.5) circle (3);
% \draw (37.1,-0.5) node {$0$};
% \draw [black] (29.7,-6.3) circle (3);
% \draw (29.7,-6.3) node {$1$};
% \draw [black] (44.9,-6.3) circle (3);
% \draw (44.9,-6.3) node {$2$};
% \draw [black] (44.9,-16.1) circle (3);
% \draw (44.9,-16.1) node {$3$};
% \draw [black] (44.9,-26) circle (3);
% \draw (44.9,-26) node {$4$};
% \draw [black] (29.7,-16.1) circle (3);
% \draw (29.7,-16.1) node {$8$};
% \draw [black] (44.9,-35.6) circle (3);
% \draw (44.9,-35.6) node {$5$};
% \draw [black] (44.9,-45.7) circle (3);
% \draw (44.9,-45.7) node {$6$};
% \draw [black] (44.9,-55.5) circle (3);
% \draw (44.9,-55.5) node {$7$};
% \draw [black] (34.74,-2.35) -- (32.06,-4.45);
% \fill [black] (32.06,-4.45) -- (33,-4.35) -- (32.38,-3.56);
% \draw (20.47,-2.9) node [above] {bfCred|unassigned};
% \draw [black] (39.51,-2.29) -- (42.49,-4.51);
% \fill [black] (42.49,-4.51) -- (42.15,-3.63) -- (41.55,-4.43);
% \draw (51,-2.9) node [above] {netDOS|http(s)};
% \draw [black] (44.9,-9.3) -- (44.9,-13.1);
% \fill [black] (44.9,-13.1) -- (45.4,-12.3) -- (44.4,-12.3);
% \draw (45.4,-11.2) node [right] {infoD|http(s)};
% \draw [black] (44.9,-19.1) -- (44.9,-23);
% \fill [black] (44.9,-23) -- (45.4,-22.2) -- (44.4,-22.2);
% \draw (45.4,-21.05) node [right] {surf|http(s)};
% \draw [black] (29.7,-9.3) -- (29.7,-13.1);
% \fill [black] (29.7,-13.1) -- (30.2,-12.3) -- (29.2,-12.3);
% \draw (29.2,-11.2) node [left] {vulnD|storage};
% \draw [black] (44.9,-29) -- (44.9,-32.6);
% \fill [black] (44.9,-32.6) -- (45.4,-31.8) -- (44.4,-31.8);
% \draw (45.4,-30.8) node [right] {vulnD|storage};
% \draw [black] (44.9,-38.6) -- (44.9,-42.7);
% \fill [black] (44.9,-42.7) -- (45.4,-41.9) -- (44.4,-41.9);
% \draw (45.4,-40.65) node [right] {serD|unassigned};
% \draw [black] (44.9,-48.7) -- (44.9,-52.5);
% \fill [black] (44.9,-52.5) -- (45.4,-51.7) -- (44.4,-51.7);
% \draw (45.4,-50.6) node [right] {hostD|http(s)};
% \end{tikzpicture}
% } %
% \hfill %
% \subcaptionbox{Attack Paths in iterated model. \label{fig:merged-paths-2-b}}
% {
% \begin{tikzpicture}[scale=0.12]
% \tikzstyle{every node}+=[inner sep=0pt]
% \draw [black] (37.5,-5.3) circle (3);
% \draw (37.5,-5.3) node {$0$};
% \draw [black] (29.7,-13.1) circle (3);
% \draw (29.7,-13.1) node {$1$};
% \draw [black] (44.9,-13.1) circle (3);
% \draw (44.9,-13.1) node {$2$};
% \draw [black] (44.9,-22.9) circle (3);
% \draw (44.9,-22.9) node {$3$};
% \draw [black] (44.9,-32.6) circle (3);
% \draw (44.9,-32.6) node {$4$};
% \draw [black] (29.7,-38.3) circle (3);
% \draw (29.7,-38.3) node {$5$};
% \draw [black] (29.7,-48.3) circle (3);
% \draw (29.7,-48.3) node {$6$};
% \draw [black] (29.7,-59.3) circle (3);
% \draw (29.7,-59.3) node {$7$};
% \draw [black] (35.38,-7.42) -- (31.82,-10.98);
% \fill [black] (31.82,-10.98) -- (32.74,-10.77) -- (32.03,-10.06);
% \draw (21.66,-8.72) node [above] {bfCred|unassigned};
% \draw [black] (39.56,-7.48) -- (42.84,-10.92);
% \fill [black] (42.84,-10.92) -- (42.65,-10) -- (41.92,-10.69);
% \draw (41.73,-7.73) node [right] {netDOS|http(s)};
% \draw [black] (44.9,-16.1) -- (44.9,-19.9);
% \fill [black] (44.9,-19.9) -- (45.4,-19.1) -- (44.4,-19.1);
% \draw (45.4,-18) node [right] {infoD|http(s)};
% \draw [black] (44.9,-25.9) -- (44.9,-29.6);
% \fill [black] (44.9,-29.6) -- (45.4,-28.8) -- (44.4,-28.8);
% \draw (45.4,-27.75) node [right] {surf|http(s)};
% \draw [black] (42.09,-33.65) -- (32.51,-37.25);
% \fill [black] (32.51,-37.25) -- (33.43,-37.43) -- (33.08,-36.5);
% \draw (43,-36.09) node [below] {vulnD|storage};
% \draw [black] (29.7,-16.1) -- (29.7,-35.3);
% \fill [black] (29.7,-35.3) -- (30.2,-34.5) -- (29.2,-34.5);
% \draw (29.2,-25.7) node [left] {vulnD|storage};
% \draw [black] (29.7,-41.3) -- (29.7,-45.3);
% \fill [black] (29.7,-45.3) -- (30.2,-44.5) -- (29.2,-44.5);
% \draw (29.2,-43.3) node [left] {serD|unassigned};
% \draw [black] (29.7,-51.3) -- (29.7,-56.3);
% \fill [black] (29.7,-56.3) -- (30.2,-55.5) -- (29.2,-55.5);
% \draw (30.2,-53.8) node [right] {hostD|http(s)};
% \end{tikzpicture}
% } %

% \caption{TODO}
% \label{fig:merged-paths-2}
% \end{figure}




